Limit laws for self-loops and multiple edges in the configuration model

We consider self-loops and multiple edges in the configuration model as the size of the graph tends to infinity. The interest in these random variables is due to the fact that the configuration model, conditioned on being simple, is a uniform random graph with prescribed degrees. Simplicity corresponds to the absence of self-loops and multiple edges. We show that the number of self-loops and multiple edges converges in distribution to two independent Poisson random variables when the second moment of the empirical degree distribution converges. We also provide an estimate on the total variation distance between the number of self-loops and multiple edges and the Poisson limit of their sum. This revisits previous works of Bollob\'as, of Janson, of Wormald and others. The error estimates also imply sharp asymptotics for the number of simple graphs with prescribed degrees. The error estimates follow from an application of Stein's method for Poisson convergence, which is a novel method for this problem. The asymptotic independence of self-loops and multiple edges follows from a Poisson version of the Cram\'er-Wold device using thinning, which is of independent interest. When the degree distribution has infinite second moment, our general results break down. We can, however, prove a central limit theorem for the number of self-loops, and for the multiple edges between vertices of degrees much smaller than the square root of the size of the graph, or when we truncate the degrees similarly. Our results and proofs easily extend to directed and bipartite configuration models.

==> header.tex <==

\RequirePackage[OT1]{fontenc}
\RequirePackage{amsthm,amssymb,amsmath}
\RequirePackage[numbers]{natbib}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{boxedminipage}
\usepackage{eepic}
%\usepackage{cprotect}
%\usepackage{math}


\oddsidemargin -8mm
\evensidemargin -8mm
\topmargin -4mm
%\headheight 4mm
%\headsep 3mm
\textheight 650pt
\textwidth 500pt


\usepackage{mathrsfs}
%\usepackage[foot]{amsaddr}
\usepackage{amssymb,amsthm,amsfonts,amsbsy,latexsym,dsfont}
%\usepackage[textsize=small]{todonotes}       % includes TO DO LIST
\usepackage{graphicx}
\usepackage[usenames,dvipsnames]{xcolor}
%\usepackage[numeric,initials,nobysame]{amsrefs}
%\usepackage{upref,setspace}
%\usepackage{natbib}
\usepackage{todonotes}
\usepackage{enumerate}
\newenvironment{enumeratei}{\begin{enumerate}[\upshape (i)]}{\end{enumerate}}
\newenvironment{enumeratea}{\begin{enumerate}[\upshape (a)]}{\end{enumerate}}
\newenvironment{enumeraten}{\begin{enumerate}[\upshape 1.]}{\end{enumerate}}
\newenvironment{enumerateA}{\begin{enumerate}[\upshape (A)]}{\end{enumerate}}
\newcommand{\RvdH}[1]{\todo[color=Magenta, inline]{Remco: #1}}
\newcommand{\CH}[1]{\todo[color=red, inline]{Cecilia: #1}}
\newcommand{\OA}[1]{\todo[color=SeaGreen, inline]{Omer: #1}}
\newcommand{\KP}[1]{\todo[inline]{Kostas: #1}}

%\submission{2013}

% 
% % settings
% \pubyear{2013}
% \volume{Submitted}
% % \issue{0}
% % \firstpage{1}
% % \lastpage{8}

\startlocaldefs


\def\UseSection{%%
        \numberwithin{equation}{section}
    \theoremstyle{plain}% default theorem style
        \newtheorem{theorem}    {Theorem}[section]
        \DefineTheorems % Use this to define other environments to be
                % numbered as ``theorem.''
}

\def\DefineTheorems{
\newtheorem{thm}[theorem]{Theorem}%[section]
\newtheorem{rem}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}%[section]
\newtheorem{defn}[theorem]{Definition}%[section]
\newtheorem{lemma}[theorem]{Lemma}%[section]
\newtheorem{prop}[theorem]{Proposition}%[section]
\newtheorem{proposition}[theorem]{Proposition}%[section]
\newtheorem{conjecture}[theorem]{Conjecture}%[section]
\newtheorem{assumption}[theorem]{Assumption}%[section]
\newtheorem{condition}[theorem]{Condition}
}
\newtheorem{exer}{Exercise}[section]
\newtheorem{openproblem}{Open Problem}[section]

\endlocaldefs

\newcommand{\B}{{\mathbb B}}
\newcommand{\C}{{\mathbb C}}
\newcommand{\E}{{\mathbb E}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\torus}{{\mathbb T}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\Zd}{{\mathbb Z}^d}
\newcommand{\Edges}{\mathbb E}
\newcommand{\Graph}{\mathbb G}
\newcommand{\N}{\mathbb N}
\newcommand{\T}{\mathbb T}
\newcommand{\Vertices}{\Z^d}
\newcommand{\ver}{\Z^d}
\newcommand{\smallsup}[1]{{\sss(\mathrm{#1})}}
\newcommand{\CRW}[1]{c^{\smallsup{RW}}_{#1}}
\newcommand{\tb}{\bar{b}}
\newcommand{\bb}{\underline{b}}
\newcommand{\olb}{\overline{b}}
\newcommand{\ulb}{\underline{b}}

\newcommand{\Gcal}{\mathscr{G}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}

\newcommand{\Comp}{\mathrm{Comp}}


\newcommand{\gr}{G}

\newcommand{\cn}{2d}
\newcommand{\bigo}{{\mathcal O}}
\newcommand{\e}{{\mathrm e}}
\renewcommand{\i}{{\mathrm i}}
\newcommand{\nnb}{\nonumber\\}
\newcommand{\AND}{~\&~}
\newcommand{\nin}{\not\in}
\newcommand{\shift}{\!\!\!\!}
%\newcommand{\const}{\mathrm{const}}
%\newcommand{\sss}{\scriptscriptstyle}


% Hatted fonts, Upper case %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Ahat} {{\hat{A} }}
\newcommand{\Bhat} {{\hat{B} }}
\newcommand{\Chat} {{\hat{C} }}
\newcommand{\Dhat} {{\hat{D} }}
\newcommand{\Ehat} {{\hat{E} }}
\newcommand{\Fhat} {{\hat{F} }}
\newcommand{\Ghat} {{\hat{G} }}
\newcommand{\Hhat} {{\hat{H} }}
\newcommand{\Ihat} {{\hat{I} }}
\newcommand{\Jhat} {{\hat{J} }}
\newcommand{\Khat} {{\hat{K} }}
\newcommand{\Lhat} {{\hat{L} }}
\newcommand{\Mhat} {{\hat{M} }}
\newcommand{\Nhat} {{\hat{N} }}
\newcommand{\Ohat} {{\hat{O} }}
\newcommand{\Phat} {{\hat{P} }}
\newcommand{\Qhat} {{\hat{Q} }}
\newcommand{\Rhat} {{\hat{R} }}
\newcommand{\Shat} {{\hat{S} }}
\newcommand{\That} {{\hat{T} }}
\newcommand{\Uhat} {{\hat{U} }}
\newcommand{\Vhat} {{\hat{V} }}
\newcommand{\What} {{\hat{W} }}
\newcommand{\Xhat} {{\hat{X} }}
\newcommand{\Yhat} {{\hat{Y} }}
\newcommand{\Zhat} {{\hat{Z} }}



%\input{preamble}

% Percolation definitions
\newcommand{\conn}{\longrightarrow}
\newcommand{\connop}{\longrightarrow}
\newcommand{\connone}{\longleftrightarrow^{1}}
\newcommand{\dis}{\displaystyle}
\newcommand{\dbc}{\Longleftrightarrow}
\newcommand{\ct}[1]     { \stackrel{#1}{\conn} }
\newcommand{\dbct}[1]     { \stackrel{#1}{\dbc} }
\newcommand{\ctx}[1]     {\leftarrow\shift\!\xrightarrow{#1}}
\newcommand{\nc}        { \conn {\hspace{-2.8ex} /} \hspace{1.8ex}   }
\newcommand{\ndbc}      {{ \, \dbc {\hspace{-3.2ex} /} \hspace{+2.0ex} }}
\newcommand{\nct}[1]     { \stackrel{#1}{\conn} {\hspace{-2.8ex} /} \hspace{1.8ex}}
\newcommand{\cdbc}[1]     { \stackrel{#1}{\dbc} }
\newcommand{\Cmax}{\mathscr{C}_{\rm max}}
\newcommand{\cluster}{\mathscr{C}}




% Definitions random graphs
\newcommand{\Ver}{U}
\newcommand{\bfwit}{\boldsymbol{w}}
\newcommand{\bfdit}{\boldsymbol{d}}
\newcommand{\bfpit}{\boldsymbol{p}}
\newcommand{\bfqit}{\boldsymbol{q}}


\newcommand{\ER}{{\rm ER}}
\newcommand{\ERnp}{{\rm ER}_n(p)}
\newcommand{\ERnq}{{\rm ER}_n(q)}
\newcommand{\ERnl}{{\rm ER}_n(\lambda/n)}
\newcommand{\GRGnw}{{\rm GRG}_n(\bfwit)}
\newcommand{\GRGnW}{{\rm GRG}_n(\mathbf{W})}
\newcommand{\CLnw}{{\rm CL}_n(\bfwit)}
\newcommand{\CLntilw}{{\rm CL}_n(\tilde{\bfwit})}
\newcommand{\CLnW}{{\rm CL}_n(\mathbf{W})}
\newcommand{\NRnw}{{\rm NR}_n(\bfwit)}
\newcommand{\NRnW}{{\rm NR}_n(\mathbf{W})}
\newcommand{\CMnd}{{\rm CM}_n(\boldsymbol{d})}
\newcommand{\DCMnd}{{\rm DCM}_n(\boldsymbol{d}^{\mathrm{\sss(in)}}, \boldsymbol{d}^{\mathrm{\sss(out)}})}
\newcommand{\BCMnd}{{\rm BCM}_n(\boldsymbol{d}^{\mathrm{\sss(l)}},\boldsymbol{d}^{\mathrm{\sss(r)}})}
\newcommand{\Confnd}{{\rm Conf}_n(\mathbf{d})}
\newcommand{\CMnD}{{\rm CM}_n(\mathbf{D})}
\newcommand{\IRGnp}{{\rm IRG}_n({\mathbf p})}
\newcommand{\IRGnq}{{\rm IRG}_n({\mathbf q})}
\newcommand{\Bin}{{\sf Bin}}
\newcommand{\Po}{{\sf Po}}
\newcommand{\sT}{{\sss \mathbb{T}}}
\newcommand{\clusterZ}{\cluster_{\sss \Z}}
\newcommand{\clusterT}{\cluster_{\sss \T}}

\newcommand{\epsn}{\varepsilon_n}

\newcommand{\Law}{\mathcal{L}}
\newcommand{\dtv}[1]{\|#1\|_{\sss \mathrm{TV}}}
\newcommand{\muX}{\mu_{\sss X}}
\newcommand{\muY}{\mu_{\sss Y}}
\newcommand{\dmax}{d_{\mathrm{max}}}
\newcommand{\Nself}{N_{\mathrm{self}}}

\def\1{{\mathchoice {1\mskip-4mu\mathrm l}      % Blackboard bold 1
{1\mskip-4mu\mathrm l}
{1\mskip-4.5mu\mathrm l} {1\mskip-5mu\mathrm l}}}
\newcommand{\indic}[1]{\1_{\{#1\}}}
\newcommand{\indicwo}[1]{\1_{#1}}

\newcommand {\convd}{\stackrel{d}{\longrightarrow}}
\newcommand {\convp}{\stackrel{\sss {\mathbb P}}{\longrightarrow}}
\newcommand {\convas}{\stackrel{a.s.}{\longrightarrow}}

\newcommand{\expec}{\mathbb{E}}
\newcommand{\prob}{\mathbb{P}}
\newcommand{\EE}{\mathcal{E}}
\newcommand{\sss}{\scriptscriptstyle}
\newcommand{\Var}{{\rm Var}}
\newcommand{\op}{o_{\sss \prob}}
\newcommand{\Op}{O_{\sss \prob}}
\newcommand{\nn}{\nonumber}

\newcommand{\Xn}{X^{\sss(n)}}
\newcommand{\Yn}{Y^{\sss(n)}}
\newcommand{\Zn}{Z^{\sss(n)}}
\newcommand{\alphan}{\alpha^{\sss(n)}}
\newcommand{\Mn}{M^{\sss(n)}}
\newcommand{\muXn}{\mu_{\sss X^{\sss(n)}}}
\newcommand{\muYn}{\mu_{\sss Y^{\sss(n)}}}
\newcommand{\lambdanS}{\lambda_n^{\sss S}}
\newcommand{\lambdanM}{\lambda_n^{\sss M}}

\newcommand{\hS}{\sss S}
\newcommand{\hM}{\sss M}
\newcommand{\bM}{\sss M}




\newcommand{\eqn}[1]{\begin{equation}#1\end{equation}}
\newcommand{\eqan}[1]{\begin{align}#1\end{align}}

